On Computationally Efficient Learning of Exponential Family Distributions

We consider the classical problem of learning, with arbitrary accuracy, the natural parameters of a $k$-parameter truncated \textit{minimal} exponential family from i.i.d. samples in a computationally and statistically efficient manner. We focus on the setting where the support as well as the natural parameters are appropriately bounded. While the traditional maximum likelihood estimator for this class of exponential family is consistent, asymptotically normal, and asymptotically efficient, evaluating it is computationally hard. In this work, we propose a novel loss function and a computationally efficient estimator that is consistent as well as asymptotically normal under mild conditions. We show that, at the population level, our method can be viewed as the maximum likelihood estimation of a re-parameterized distribution belonging to the same class of exponential family. Further, we show that our estimator can be interpreted as a solution to minimizing a particular Bregman score as well as an instance of minimizing the \textit{surrogate} likelihood. We also provide finite sample guarantees to achieve an error (in $\ell_2$-norm) of $\alpha$ in the parameter estimation with sample complexity $O({\sf poly}(k)/\alpha^2)$. Our method achives the order-optimal sample complexity of $O({\sf log}(k)/\alpha^2)$ when tailored for node-wise-sparse Markov random fields. Finally, we demonstrate the performance of our estimator via numerical experiments.

==> content/conclusion.tex <==
\section{Conclusion}
We provide rigorous finite sample analysis for learning structure and parameters of continuous MRFs without the abstract conditions of incoherence, dependency, sparse eigenvalue or restricted strong convexity that are common in literature. We provide easy-to-verify sufficient condition for learning that is naturally satisfied for polynomial and harmonic sufficient statistics. Our methodology requires $\bcO(p^{2})$ computations and $O(\exp(d)\log p)$ samples similar to the discrete and Gaussian settings. Additionally, we propose a robust variation of Lasso by showing that even in the presence of bounded additive noise, the Lasso estimator is ‘prediction consistent’ under mild assumptions.

We also establish that minimizing the population version of GISO \cite{VuffrayML2019} is equivalent to finding MLE of a certain related parametric distribution. We provide asymptotic consistency and normality of the estimator under mild conditions. Further, we show that the GISO is equivalent to the surrogate likelihood proposed by Jeon et al. (2006) \cite{JeonL2006}.

A natural extension of the pairwise setup is the $t$-wise MRF with continuous variables. The approach and the objective function introduced in Vuffray et al. (2019) \cite{VuffrayML2019} naturally extend for such a setting allowing to learn $t$-wise MRFs with general discrete variables as explained in that work. We believe that our results for continuous setting, in a similar vein, extend for $t$-wise MRFs as well and it is an important direction for immediate future work. We also believe that the connection of the GISO to KL-divergence could be used to remove the bounded random variables assumption of our work. Another important direction is to leverage the asymptotic normality of the estimator established in our work to construct data-driven explicit confidence intervals for learned parameters of MRF.
